A Backend Framework for the Efficient Management of Power System Measurements

Increased adoption and deployment of phasor measurement units (PMU) has provided valuable fine-grained data over the grid. Analysis over these data can provide insight into the health of the grid, thereby improving control over operations. Realizing this data-driven control, however, requires validating, processing and storing massive amounts of PMU data. This paper describes a PMU data management system that supports input from multiple PMU data streams, features an event-detection algorithm, and provides an efficient method for retrieving archival data. The event-detection algorithm rapidly correlates multiple PMU data streams, providing details on events occurring within the power system. The event-detection algorithm feeds into a visualization component, allowing operators to recognize events as they occur. The indexing and data retrieval mechanism facilitates fast access to archived PMU data. Using this method, we achieved over 30x speedup for queries with high selectivity. With the development of these two components, we have developed a system that allows efficient analysis of multiple time-aligned PMU data streams.

==> bios.tex <==
\begin{IEEEbiographynophoto}
{Ben McCamish}
is completing his Ph.D.~in Computer Science at Oregon State University. His research interests include large scale data management and artificial intelligence design. 
\vspace{-0.50in}
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}
{Rich Meier}
is completing his Master's in Electrical and Computer Engineering at Oregon State University.
\vspace{-0.48in}
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}
{Jordan Landford}
is pursuing his M.S.~in Electrical and Computer Engineering at Portland State University.
\vspace{-0.48in}
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}
{Robert Bass} received the Ph.D.~degree in electrical engineering in 2004 from The University of Virginia. Currently, he is Associate Professor in the School of Electrical \& Computer Engineering at Portland State University, Portland, OR, USA. His research interests pertain to electric power distribution assets, power quality, renewables integration and distributed energy storage systems.
\vspace{-0.44in}
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}
{Eduardo Cotilla-Sanchez} received the Ph.D.~degree in electrical engineering in 2012 from The University of Vermont. He is currently an Assistant Professor in the School of Electrical Engineering \& Computer Science at Oregon State University. His primary field of research is the vulnerability of electrical infrastructure, in particular, the study of cascading outages. Cotilla-Sanchez is the Secretary of the IEEE Cascading Failure Working Group and President of SHPE Oregon Chapter. 
\vspace{-0.44in}
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}
{David Chiu} received a Ph.D.~in computer science and engineering in 2010 from The Ohio State University. He is an Assistant Professor of Computer Science at the University of Puget Sound. His research interests include large-scale data management and data-intensive processing.
\end{IEEEbiographynophoto}


==> preamble.tex <==
\renewcommand{\dbltopfraction}{0.85}
%\renewcommand{\dblfloatpagefraction}{.85}
% \newcommand{\comment}[1]{}

%\raggedbottom

\hyphenation{Post-Order Reverse-Post-Order Pre-Order Reverse-Pre-Order}

% -------------------------------------------------------------
% RvH 11/17/91; Commands for lining up code samples

\newsavebox{\boxone}
\newsavebox{\boxtwo}
\newsavebox{\boxthree}

\newlength{\narrow}
\setlength{\narrow}{.45\textwidth}
\newlength{\cnarrow}
\setlength{\cnarrow}{.45\columnwidth}

\newcommand{\topline}{
  \hrule
  \vskip .5\baselineskip}
\newcommand{\bottomline}{
  \vskip 2pt
  \hrule}

% produces centered horizontal box
% #1 = width, #2 = box contents
\newcommand{\chbox}[2]{
  \hbox to #1{\hss\vtop{#2}\hss}}

% produces centered narrow box
% #1 = box contents
\newcommand{\nchbox}[1]{
  \chbox{\narrow}{#1}}

% produces centered cnarrow box
% #1 = box contents
\newcommand{\cnchbox}[1]{
  \chbox{\cnarrow}{#1}}

% produces centered code
% #1 = file with TeX'ed code, #2 = desired width
\newcommand{\code}[2]{
  \chbox{#1}{\tgrind\input{#2}}}

% produces code of full text width
% #1 = file with TeX'ed code
\newcommand{\fcode}[1]{
  \code{\textwidth}{#1}}

% produces narrow code
% #1 = file with TeX'ed code
\newcommand{\ncode}[1]{
  \code{\narrow}{#1}}

% produces narrow figure
% #1 = figure, #2 = caption, #4 = label
\def\nfig#1#2#3{
  \vtop{\nchbox{#1}
  \hbox to\narrow{\parbox{\narrow}{\caption{#2}\label{#3}}}}}

% produces narrow code figure
% #1 = file, #2 = caption, #4 = label
\def\ncodefig#1#2#3{
  \nfig{\ncode{#1}}{#2}{#3}}

% produces cnarrow code
% #1 = file with TeX'ed code
\newcommand{\cncode}[1]{\code{\cnarrow}{#1}}

\def\codefiggen[#1]#2#3#4#5#6{
  \begin{figure}[#1]
  #5
  \fcode{#2}
  \center\parbox{.9\textwidth}{\caption{#3}\label{#4}}
  #6
  \end{figure}}

% Create one code figure
% #1 = loc, #2 = file, #3 = caption, #4 = label
\def\codefig[#1]#2#3#4{
  \codefiggen[#1]{#2}{#3}{#4}{}{}}

% Create one code figure, with lines
% #1 = loc, #2 = file, #3 = caption, #4 = label
\def\codefigline[#1]#2#3#4{
  \codefiggen[#1]{#2}{#3}{#4}{\topline}{\bottomline}}

\def\doublefiggen[#1]#2#3#4#5#6#7#8#9{
  \begin{figure}[#1]
  #8
  \hbox to \textwidth{
  \nfig{#2}{#3}{#4}
  \hfil
  \nfig{#5}{#6}{#7}}
  #9
  \end{figure}}

% Creates two figures, side by side
% #1 = loc, #2 = fig1, #3 = caption1, #4 = label1, #5 = fig2, 
% #6 = caption2, #7 = label2
\def\doublefig[#1]#2#3#4#5#6#7{
  \doublefiggen[#1]{#2}{#3}{#4}{#5}{#6}{#7}{}{}}

% Creates two figures, side by side, with lines
% #1 = loc, #2 = fig1, #3 = caption1, #4 = label1, #5 = fig2, 
% #6 = caption2, #7 = label2
\def\doublefigline[#1]#2#3#4#5#6#7{
  \doublefiggen[#1]{#2}{#3}{#4}{#5}{#6}{#7}{\topline}{\bottomline}}

% Creates two code figures, side by side
% #1 = loc, #2 = code1, #3 = caption1, #4 = label1, #5 = code2, 
% #6 = caption2, #7 = label2
\def\doublecodefig[#1]#2#3#4#5#6#7{
  \doublefig[#1]{\ncode{#2}}{#3}{#4}{\ncode{#5}}{#6}{#7}}

% Creates two code figures, side by side, with lines
% #1 = loc, #2 = code1, #3 = caption1, #4 = label1, #5 = code2, 
% #6 = caption2, #7 = label2
\def\doublecodefigline[#1]#2#3#4#5#6#7{
  \doublefigline[#1]{\ncode{#2}}{#3}{#4}{\ncode{#5}}{#6}{#7}}

% #1 = file1, #2 = caption1, #3 = file2, #4 = caption2
\newcommand{\codepair}[4]{\vbox{
  \hbox{\ncode{#1} \hfil \ncode{#3}}
  \vskip .3\baselineskip plus .3\baselineskip
  \hbox{\hbox to\narrow{#2\hfil} \hfil \hbox to\narrow{#4\hfil}}}}

% Creates one figure with two codes, side by side
% #1 = loc, #2 = file1, #3 = caption1, #4 = file2, #5 = caption2, 
% #6 = caption, #7 = label 
\def\codepairfig[#1]#2#3#4#5#6#7{
  \begin{figure}[#1]
  \codepair{#2}{#3}{#4}{#5}
  \center\parbox{.9\textwidth}{\caption{#6}}
  \label{#7}
  \end{figure}}

\def\cncodepairfiggen[#1]#2#3#4#5#6#7{
  \begin{figure}[#1]
  #6
  \hbox{\cncode{#2}\hfil\cncode{#3}}
  \center\parbox{.9\columnwidth}{\caption{#4}\label{#5}}
  #7
  \end{figure}}

% Create one narrow figure with 1 caption, 2 codes
% #1 = loc, #2 = file1, #3 = file2, #4 = caption, #5 = label
\def\cncodepairfig[#1]#2#3#4#5{
  \cncodepairfiggen[#1]{#2}{#3}{#4}{#5}{}{}}

% Create one narrow figure with 1 caption, 2 codes, with lines
% #1 = loc, #2 = file1, #3 = file2, #4 = caption, #5 = label
\def\cncodepairfigline[#1]#2#3#4#5{
  \cncodepairfiggen[#1]{#2}{#3}{#4}{#5}{\topline}{\bottomline}}

% Create two figures with one caption
% #1 = loc, #2 = fig1, #3 = fig2, #4 = caption, #5 = label
\def\doublefigOnecap*[#1]#2#3#4#5{
  \begin{figure*}[#1]
  \hbox to \textwidth{
  \nchbox{#2}
  \hfil
  \nchbox{#3}}
  \caption{#4}
  \label{#5}
  \end{figure*}}

% Create two figures with one caption
% #1 = loc, #2 = fig1, #3 = fig2, #4 = caption, #5 = label
\def\doublefigOnecap[#1]#2#3#4#5{
  \begin{figure}[#1]
  \topline
  \hbox to \columnwidth{
  \cnchbox{#2}
  \hfil
  \cnchbox{#3}}
  \caption{#4}
  \label{#5}
  \bottomline
  \end{figure}}

% Create one figure with one postscript file
% #1 = loc, #2 = ps, #3 = caption, #4 = label
\def\PSfig[#1]#2#3#4{
 \begin{figure}
 \centerline{\psfig{file=#2,width=\columnwidth}}
 \caption{{#3}} 
 \label{#4}
 \end{figure}}

% Create one figure with one postscript file, with lines
% #1 = loc, #2 = ps, #3 = caption, #4 = label
\def\PSfiglines[#1]#2#3#4{
 \begin{figure}[#1]
 \topline
 \centerline{\psfig{file=#2,width=\columnwidth}}
 \caption{{#3}} 
 \label{#4}
 \bottomline
 \end{figure}}

% Create one figure with one postscript file, with lines
% #1 = loc, #2 = ps, #3 = caption, #4 = label
\def\PSfiglinesht[#1]#2#3#4#5{
 \begin{figure}[#1]
 \topline
 \centerline{\psfig{file=#2,height=#3}}
 \caption{{#4}} 
 \label{#5}
 \bottomline
 \end{figure}}

% Create one figure with two postscript files, side by side
% #1 = loc, #2 = ps1, #3 = ps2, #4 = height, #5 = caption, #6 = label
\def\doublePSfig[#1]#2#3#4#5#6{
  \doublefigOnecap[#1]
    {\cnchbox{\psfig{file=#2,height=#4}}}
    {\cnchbox{\psfig{file=#3,height=#4}}}
    {#5}
    {#6}}

% Keywords
\def\k#1{{\bf #1}}
\def\m#1{{\em #1}}
\def\f#1{{\sf #1}}

\newlength{\boxwidth}
\setlength{\boxwidth}{3.2in}

\newcommand{\bproof}{{\bf Proof:}}
\newcommand{\eproof}{\mbox{$\Box$}}
\newcommand{\ind}{\; + \; {\em induction}}

% Environment for codes based on \tabbing
\def\tabcodeold#1#2#3{%
\begin{figure}[t]%
\hrule%
%\bcenter
%\framebox[\boxwidth]{
\center\parbox{\boxwidth}{%
\vbox{%
\begin{tabbing}%
#1
\end{tabbing}}}
 %\ecenter
 \caption{#2\label{#3}}
 \bottomline
 \end{figure}
}

% Environment for codes based on \tabbing
\def\tabcode#1#2#3{
 \begin{figure}[tbh]
 \topline\vs{-.4}
 \center{\begin{minipage}{\boxwidth}
 \small
 \begin{tabbing}
 #1
 \end{tabbing}
 \end{minipage}}
 \caption{#2\label{#3}}
 \bottomline
 \end{figure}
} 

\def\tabcodenoline#1#2#3{
 \begin{figure}[tbh]
 \center{\begin{minipage}{\boxwidth}
 \small
 \begin{tabbing}
 #1
 \end{tabbing}
 \end{minipage}}
 \caption{#2\label{#3}}
 \end{figure}
} 

% Command for putting a frame around a piece of code
\def\fboxcode#1{%
 \small
 \fbox{%
 \begin{minipage}{\textwidth}
 \begin{tabbing}
 \tab\=\tab\=\tab\=\kill
 #1
 \end{tabbing}
 \end{minipage}}}

% Environment for two columns of code, based on \tabbing
\def\tabdoublecode#1#2#3#4{
 \begin{figure*}[t]
 \topline\vs{-.4}
 \hbox to \columnwidth{
 \vtop{\small
 \begin{tabbing}
 #1
 \end{tabbing}}
 \hfil
 \hfil
 \hfil
 \vtop{\small
 \begin{tabbing}
 #2
 \end{tabbing}}
 }
 \caption{#3\label{#4}}
 \bottomline
 \end{figure*}
}
\def\tabtriplecode#1#2#3#4#5{
 \begin{figure}
 \topline\vs{-.4}
 \hbox to \columnwidth{
 \vtop{\small
 \begin{tabbing}
 #1
 \end{tabbing}}
 \hfil
 \hfil
 \hfil
 \vtop{\small
 \begin{tabbing}
 #2
 \end{tabbing}}
 \hfil
 \hfil
 \hfil
 \vtop{\small
 \begin{tabbing}
 #3
 \end{tabbing}}
 }
 \caption{#4\label{#5}}
 \bottomline
 \end{figure}
}


% -------------------------------------------------------------

% Referencing and labelling
\newcommand{\lr}[1]{\label{ded:#1}}
\newcommand{\dr}[1]{(\ref{ded:#1})}
\newcommand{\er}[1]{(\ref{eq:#1})}
\newcommand{\eqq}[1]{\ref{eq:#1}}

\newcommand{\eqby}[1]{{\stackrel{#1}{=}}}
\newcommand{\supseteqby}[1]{{\st}ackrel{#1}{\supseteq}}
\newcommand{\by}[1]{{\stackrel{#1}{\longrightarrow}}}
\newcommand{\byr}[1]{\by{\er{#1}}}
\newcommand{\byl}[1]{\by{\dr{#1}}}
\newcommand{\eqbyr}[1]{\eqby{\er{#1}}}

% Environment for deductions
\def\ded#1#2#3#4{
 \begin{equation}
 \lr{#1}
 [#2] \;\;\; \by{#3} \;\;\; {#4}
 \end{equation}}

% Environment for facts
\newcommand{\fac}[2]{
 \begin{equation}
 \label{ded:#1}
 {#2}
 \end{equation}}

% Negating
\def\no#1{\overline{#1}}

%Environment for lemmata, theorems



% -------------------------------------------------------------

\newcommand{\naive}{{na\"{\i}ve}}
\newcommand{\naively}{{na\"{\i}vely}}

\def\FortD{{Fortran~D}}
\def\FssD{{Fortran 77D}}
\def\FnineD{{Fortran 90D}}
\def\Parti{{\sc Parti}}

\newcommand{\order}[1]{\mbox{${\cal O}(#1)$}}
\newcommand{\eg}{{\em e.g.}}
\newcommand{\Eg}{{\em E.g.}}
\newcommand{\ie}{{\em i.e.}}
%\def\etal{{\em et~al.}}
\def\etal{et~al.~}
\newcommand{\eqv}{\mbox{ $\equiv$ }}
\newcommand{\lp}{\mbox{\bf (}}
\newcommand{\rp}{\mbox{\bf )}}
\newcommand{\sla}{\mbox{ $\leftarrow$ }}
\newcommand{\la}{\mbox{ $\longleftarrow$ }}
\newcommand{\La}{\mbox{ $\Longleftarrow$ }}
\newcommand{\ra}{\mbox{ $\longrightarrow$ }}
\newcommand{\ar}{\mbox{ $\rightarrow$ }}
\newcommand{\Ra}{\mbox{ $\Longrightarrow$ }}
\newcommand{\Lra}{\mbox{ $\Leftrightarrow$ }}
\newcommand{\LLra}{\mbox{ $\Longleftrightarrow$ }}
%\newcommand{\caupspace}{\!\!\!}
\newcommand{\caupspace}{\!\!\!}
\newcommand{\tight}[1]{\hs{-.02in}#1\hs{-.04in}}
\newcommand{\bgcap}[1]{\displaystyle\caupspace\bigcap_{#1}\caupspace}
\newcommand{\bgcup}[1]{\displaystyle\caupspace\bigcup_{#1}\caupspace}
\newcommand{\req}{&\caupspace=\caupspace&}
\newcommand{\hs}[1]{\hspace{#1}}
\newcommand{\tab}{\hs{.2in}}
\newcommand{\vs}[1]{\vspace{#1cm}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bec}[1]{\setcounter{equation}{#1} \be}
\newcommand{\through}{\mbox{$:$}}
\newcommand{\eqr}[2]{\mbox{$E(\ref{eq:#1}, #2)$}}

\newcommand{\bdesc}{\begin{description}}
\newcommand{\edesc}{\end{description}}
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}
\newcommand{\bitem}{\begin{itemize}}
\newcommand{\eitem}{\end{itemize}}
\newcommand{\bcenter}{\begin{center}}
\newcommand{\ecenter}{\end{center}}
\newcommand{\btabular}{\begin{tabular}}
\newcommand{\etabular}{\end{tabular}}
\newcommand{\beqnarr}{
 %\setlength{\jot}{1pt}
 %\setlength{\abovedisplayskip}{0ex}
 \begin{eqnarray}}
\newcommand{\eeqnarr}{\end{eqnarray}}
 
\newcommand{\bnf}[1]{$\langle {#1} \rangle$}
 
\newcommand{\port}[1]{\hat{#1}}
\newcommand{\eltaccent}[1]{\tilde{#1}}
\newcommand{\elt}[1]{\eltaccent{#1}}
\newcommand{\eltt}[1]{\eltaccent{\eltaccent{\mbox{$#1$}}}}
\newcommand{\mysetminus}{-}
\newcommand{\mysetminuss}{\eltt{\mysetminus}}
\newcommand{\melt}[1]{\mbox{$\elt{#1}$}}
\newcommand{\meltt}[1]{\mbox{$\eltt{#1}$}}
\newcommand{\mport}[1]{\mbox{$\port{#1}$}}
\newcommand{\mmysetminuss}{\mbox{$\mysetminuss$}}
\newcommand{\cl}[1]{${\cal#1}$}
 
\newcommand{\str}[1]{{\em #1}^*}
 
\newcommand{\spread}[1]{\mbox{{\em {#1}}$^*$}}
\newcommand{\affect}[1]{\mbox{{\em {#1}}$^\cup$}}
\newcommand{\contain}[1]{\mbox{{\em {#1}}$^\cap$}}
\newcommand{\touch}[1]{\mbox{{\em {#1}}$^\circ$}}
 
\newcommand{\ALL}{\top}
\newcommand{\VAR}{\f{VAR}}
\newcommand{\BLOCK}{\f{BLOCK}}
\newcommand{\GEN}{\f{GEN}}
\newcommand{\GIVE}{\f{GIVE}}
\newcommand{\GIVEN}{\f{GIVEN}}
\newcommand{\MOVE}{\f{MOVE}}
\newcommand{\RES}{\f{RES}}
\newcommand{\STEAL}{\f{STEAL}}
\newcommand{\TAKE}{\f{TAKE}}
\newcommand{\TAKEN}{\f{TAKEN}}

\newcommand{\gt}{{\em GiveNTake}}
\newcommand{\Gtp}{Give-N-Take}
\newcommand{\Gt}{{\sc \Gtp}}
%\newcommand{\smallbf}{\small\bf}
\newcommand{\GT}{G{\small\bf IVE}-N-T{\small\bf AKE}}
\newcommand{\Eager}{\mbox{\sc Eager}}
\newcommand{\Lazy}{\mbox{\sc Lazy}}
\newcommand{\entry}{\mbox{$_{\em entry}$}}
\newcommand{\jump}{\mbox{$_{\em jump}$}}
\newcommand{\loc}{\mbox{$_{\em loc}$}}
\newcommand{\In}{{\em in}}
\newcommand{\Out}{{\em out}}
\newcommand{\inn}{\mbox{$_{\In}$}}
\newcommand{\init}{\mbox{$_{\em init}$}}
\newcommand{\out}{\mbox{$_{\Out}$}}
\newcommand{\sib}{\mbox{$_{\em siblings}$}}
\newcommand{\eeager}{{\em eager}}
\newcommand{\elazy}{{\em lazy}}
\newcommand{\earl}{\mbox{$^{\eeager}$}}
\newcommand{\eager}{\mbox{$^{\eeager}$}}
\newcommand{\eagerin}{\mbox{$^{\eeager}_{\em in}$}}
\newcommand{\eagerout}{\mbox{$^{\eeager}_{\em out}$}}
\newcommand{\lazy}{\mbox{$^{\elazy}$}}
\newcommand{\lazyin}{\mbox{$^{\elazy}_{\em in}$}}
\newcommand{\lazyout}{\mbox{$^{\elazy}_{\em out}$}}

\newcommand{\excode}{{\em prog}}
\newcommand{\Dir}{\mbox{\sc Direction}}
\newcommand{\Read}{\mbox{\sc Read}}
\newcommand{\Write}{\mbox{\sc Write}}
%\newcommand{\Send}{\mbox{$_{\sc Send}$}}
%\newcommand{\Recv}{\mbox{$_{\sc Recv}$}}
\newcommand{\Send}{\mbox{$_{\em Send}$}}
\newcommand{\Recv}{\mbox{$_{\em Recv}$}}
\newcommand{\WriteAdd}{{\sc WriteAdd}}
\newcommand{\WriteMult}{{\sc WriteMult}}
\newcommand{\Upward}{{\sc Upward}}
\newcommand{\Downward}{{\sc Downward}}
\newcommand{\Forward}{{\sc Forward}}
\newcommand{\Backward}{{\sc Backward}}
\newcommand{\Before}{{\sc Before}}
\newcommand{\After}{{\sc After}}
\newcommand{\pre}{{\sc PreOrder}}
\newcommand{\post}{{\sc PostOrder}}
\newcommand{\revpre}{{\sc ReversePreOrder}}
\newcommand{\revpost}{{\sc ReversePostOrder}}
%\newcommand{\}{{\em }}
\newcommand{\TP}{$T^+$}
\newcommand{\Children}{\mbox{\sc Children}}
\newcommand{\preds}{\mbox{\footnotesize\sc Preds}}
%\newcommand{\predsP}{\mbox{{\footnotesize\sc Preds}$^+$}}
\newcommand{\Preds}{\mbox{\sc Preds}}
%\newcommand{\PredsP}{\mbox{{\sc Preds}$^+$}}
%\newcommand{\succs}{\mbox{\footnotesize\sc Succs}}
\newcommand{\Succs}{\mbox{\sc Succs}}
%\newcommand{\succsP}{\mbox{{\footnotesize\sc Succs}$^+$}}
%\newcommand{\SuccsP}{\mbox{{\sc Succs}$^+$}}
%\newcommand{\succsM}{\mbox{{\footnotesize\sc Succs}$^-$}}
%\newcommand{\SuccsM}{\mbox{{\sc Succs}$^-$}}
\newcommand{\type}{\mbox{{\scriptsize T}{\tiny YPE}}}
\newcommand{\Type}{\mbox{\sc Type}}
\newcommand{\Back}{\mbox{\sc Cycle}}
\newcommand{\Entry}{\mbox{\sc Entry}}
\newcommand{\Flow}{\mbox{\sc Forward}}
\newcommand{\Jump}{\mbox{\sc Jump}}
\newcommand{\Synthetic}{\mbox{\sc Synthetic}}
\newcommand{\Bletter}{C}
\newcommand{\Eletter}{E}
\newcommand{\Fletter}{F}
\newcommand{\Jletter}{J}
\newcommand{\Sletter}{S}
\newcommand{\ET}{{\rm \Eletter}}
\newcommand{\BT}{{\rm \Bletter}}
\newcommand{\JT}{{\rm \Jletter}}
\newcommand{\FT}{{\rm \Fletter}}
\newcommand{\ST}{{\rm \Sletter}}
\newcommand{\Et}{{\rm\small \Eletter}}
\newcommand{\Bt}{{\rm\small \Bletter}}
\newcommand{\Jt}{{\rm\small \Jletter}}
\newcommand{\Ft}{{\rm\small \Fletter}}
\newcommand{\St}{{\rm\small \Sletter}}
\newcommand{\et}{\mbox{\tiny \Eletter}}
\newcommand{\bt}{\mbox{\tiny \Bletter}}
\newcommand{\jt}{\mbox{\tiny \Jletter}}
\newcommand{\ft}{\mbox{\tiny \Fletter}}
%\newcommand{\st}{\mbox{\tiny \Sletter}}
\newcommand{\meetees}{\mbox{\sc meetees}}
\newcommand{\Root}{\mbox{\sc Root}}
\newcommand{\Header}{\mbox{\sc Header}}
\newcommand{\Start}{\mbox{\sc Start}}
\newcommand{\Stop}{\mbox{\sc Stop}}
%\newcommand{\FirstChild}{\mbox{\sc FirstChild}}
%\newcommand{\firstChild}{\mbox{\footnotesize\sc FirstChild}}
\newcommand{\LastChild}{\mbox{\sc LastChild}}
\newcommand{\level}{\mbox{\sc Level}}

%\newcommand{\Partners}{{\em Partners}}
%\newcommand{\Pairs}{{\em Pairs}}


%% David
%%
%Symbol footnotes
\long\def\symbolfootnote[#1]#2{\begingroup
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}


\newcommand{\eat}[1]{}
\newcommand \TODO[2]{\textcolor{red}{[\textbf{#1}] #2 }}
\newcommand{\reminder}[1]{{\bf  [[  #1 ]]}\typeout{#1}}
\newcommand{\etc}{etc}

%Space saving
\newcommand{\Section}[1]{\section{#1}}
\newcommand{\SectionS}[1]{\section*{#1}}
\newcommand{\Subsection}[1]{\subsection{#1}}
\newcommand{\Subsubsection}[1]{\subsubsection{#1}}

